Constraining values of bag constant for strange star candidates

We provide a strange star model under the framework of general relativity by using a general linear equation of state (EOS). The solution set thus obtained is employed on altogether 20 compact star candidates to constraint values of MIT bag model. No specific value of the bag constant ($B$) a-priori is assumed rather possible range of values for bag constant is determined from observational data of the said set of compact stars. To do so the Tolman-Oppenheimer-Volkoff (TOV) equation is solved by homotopy perturbation method (HPM) and hence we get a mass function for the stellar system. The solution to the Einstein field equations represents a non-singular, causal and stable stellar structure which can be related to strange stars. Eventually we get an interesting result on the range of the bag constant as 41.58~MeV~fm$^{-3}< B <$319.31~MeV~fm$^{-3}$. We have found the maximum surface redshift $Z^{max}_{s}=0.63$ and shown that the central redshift ($Z_c$) can not have value larger than $2k$, where $k=2.010789 \pm 0.073203$. Also we provide a possible value of bag constant for neutron star (NS) with quark core using hadronic as well as quark EOS.

==> pifont.psy.tex <==
%%
%% This is file `pifont.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% psfonts.dtx  (with options: `pifont')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pifont.sty.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file psfonts.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\ProvidesPackage{pifont}
[2002/09/08 PSNFSS-v9.0a
Pi font support (SPQR)
]
\newcommand{\Pifont}[1]{\fontfamily{#1}\fontencoding{U}%
\fontseries{m}\fontshape{n}\selectfont}
\newcommand{\Pisymbol}[2]{{\Pifont{#1}\char#2}}
\newcommand{\Pifill}[2]{\leaders\hbox{\makebox[0.2in]{%
       \Pisymbol{#1}{#2}}}\hfill\kern\z@}
\newcommand{\Piline}[2]{\par\noindent\hspace{0.5in}\Pifill{#1}{#2}%
       \hspace{0.5in}\kern\z@\par}
\newenvironment{Pilist}[2]%
{\begin{list}{\Pisymbol{#1}{#2}}{}}%
{\end{list}}%
\def\Pinumber#1#2{\protect\Pisymbol{#1}{\arabic{#2}}}
\newenvironment{Piautolist}[2]{%
\ifnum \@enumdepth >3 \@toodeep\else
      \advance\@enumdepth \@ne
      \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
  \expandafter\def\csname p@enum\romannumeral\the\@enumdepth\endcsname{}%
  \expandafter\def\csname labelenum\romannumeral\the\@enumdepth\endcsname{%
     \csname theenum\romannumeral\the\@enumdepth\endcsname}%
  \expandafter\def\csname theenum\romannumeral\the\@enumdepth\endcsname{%
     \Pinumber{#1}{enum\romannumeral\the\@enumdepth}}%
  \list{\csname label\@enumctr\endcsname}{%
        \@nmbrlisttrue
        \def\@listctr{\@enumctr}%
        \setcounter{\@enumctr}{#2}%
        \addtocounter{\@enumctr}{-1}%
        \def\makelabel##1{\hss\llap{##1}}}
\fi
}{\endlist}
\newcommand{\ding}{\Pisymbol{pzd}}
\def\dingfill#1{\leaders\hbox{\makebox[0.2in]{\Pisymbol{pzd}{#1}}}\hfill}
\def\dingline#1{\Piline{pzd}{#1}}
\newenvironment{dinglist}[1]{\begin{Pilist}{pzd}{#1}}%
  {\end{Pilist}}
\newenvironment{dingautolist}[1]{\begin{Piautolist}{pzd}{#1}}%
  {\end{Piautolist}}
{\Pifont{pzd}}
{\Pifont{psy}}
\endinput
%%
%% End of file `pifont.sty'.

==> pifont.sty.tex <==
%%
%% This is file `pifont.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% psfonts.dtx  (with options: `pifont')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from pifont.sty.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file psfonts.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
\ProvidesPackage{pifont}
[2002/09/08 PSNFSS-v9.0a
Pi font support (SPQR)
]
\newcommand{\Pifont}[1]{\fontfamily{#1}\fontencoding{U}%
\fontseries{m}\fontshape{n}\selectfont}
\newcommand{\Pisymbol}[2]{{\Pifont{#1}\char#2}}
\newcommand{\Pifill}[2]{\leaders\hbox{\makebox[0.2in]{%
       \Pisymbol{#1}{#2}}}\hfill\kern\z@}
\newcommand{\Piline}[2]{\par\noindent\hspace{0.5in}\Pifill{#1}{#2}%
       \hspace{0.5in}\kern\z@\par}
\newenvironment{Pilist}[2]%
{\begin{list}{\Pisymbol{#1}{#2}}{}}%
{\end{list}}%
\def\Pinumber#1#2{\protect\Pisymbol{#1}{\arabic{#2}}}
\newenvironment{Piautolist}[2]{%
\ifnum \@enumdepth >3 \@toodeep\else
      \advance\@enumdepth \@ne
      \edef\@enumctr{enum\romannumeral\the\@enumdepth}%
  \expandafter\def\csname p@enum\romannumeral\the\@enumdepth\endcsname{}%
  \expandafter\def\csname labelenum\romannumeral\the\@enumdepth\endcsname{%
     \csname theenum\romannumeral\the\@enumdepth\endcsname}%
  \expandafter\def\csname theenum\romannumeral\the\@enumdepth\endcsname{%
     \Pinumber{#1}{enum\romannumeral\the\@enumdepth}}%
  \list{\csname label\@enumctr\endcsname}{%
        \@nmbrlisttrue
        \def\@listctr{\@enumctr}%
        \setcounter{\@enumctr}{#2}%
        \addtocounter{\@enumctr}{-1}%
        \def\makelabel##1{\hss\llap{##1}}}
\fi
}{\endlist}
\newcommand{\ding}{\Pisymbol{pzd}}
\def\dingfill#1{\leaders\hbox{\makebox[0.2in]{\Pisymbol{pzd}{#1}}}\hfill}
\def\dingline#1{\Piline{pzd}{#1}}
\newenvironment{dinglist}[1]{\begin{Pilist}{pzd}{#1}}%
  {\end{Pilist}}
\newenvironment{dingautolist}[1]{\begin{Piautolist}{pzd}{#1}}%
  {\end{Piautolist}}
{\Pifont{pzd}}
{\Pifont{psy}}
\endinput
%%
%% End of file `pifont.sty'.
